Dr Jekyll and Mr Hyde: the Strange Case of Off-Policy Policy Updates

The policy gradient theorem states that the policy should only be updated in states that are visited by the current policy, which leads to insufficient planning in the off-policy states, and thus to convergence to suboptimal policies. We tackle this planning issue by extending the policy gradient theory to policy updates with respect to any state density. Under these generalized policy updates, we show convergence to optimality under a necessary and sufficient condition on the updates' state densities, and thereby solve the aforementioned planning issue. We also prove asymptotic convergence rates that significantly improve those in the policy gradient literature. To implement the principles prescribed by our theory, we propose an agent, Dr Jekyll & Mr Hyde (JH), with a double personality: Dr Jekyll purely exploits while Mr Hyde purely explores. JH's independent policies allow to record two separate replay buffers: one on-policy (Dr Jekyll's) and one off-policy (Mr Hyde's), and therefore to update JH's models with a mixture of on-policy and off-policy updates. More than an algorithm, JH defines principles for actor-critic algorithms to satisfy the requirements we identify in our analysis. We extensively test on finite MDPs where JH demonstrates a superior ability to recover from converging to a suboptimal policy without impairing its speed of convergence. We also implement a deep version of the algorithm and test it on a simple problem where it shows promising results.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{They are discussed a bit everywhere and for more transparency, we inventory them in \sect{} \ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{We do not believe that there exists any potential negative societal impact that is specific of our work. We improve understanding and algorithm of one branch of RL algorithms. Like any tool, it may be used with ill-intents, and improving the tool raises the potential harm. We do not introduce new applications, new source of bias, nor new data handling processes.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All theorems are associated with the set of assumptions/conditions they depend on.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We include complete proof for the all the stated theorems in \app{} \ref{app:theory}. For the technical proofs, we also include a proof sketch to explain it at a higher level.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{It is included in the supplementary material during submission, and will be made public in case of acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We tried to do so in \app{} \ref{app:domains}, \ref{app:expes-exact}, \ref{app:expes-sample}, and \ref{app:expes-deep}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We did it only in the deep RL experiments (see \sect{} \ref{sec:expe-deep} and \app{} \ref{app:expes-deep}). In the other experiments, either there was no stochasticity at all, or we reported a figure with the decile performance in \app{}  (see \fig{} \ref{fig:exact-garnets-direct-decile}, \ref{fig:exact-garnets-softmax-decile}, and \ref{fig:sample-garnets-long_time-decile}).}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We did it for the deep RL experiments in \app{} \ref{app:expes-deep}. The finite MDP experiments were small enough not to require such details in our opinion.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite~\cite{pchrist}.}
  \item Did you mention the license of the assets?
    \answerYes{The MIT license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{It is included in the code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Not applicable.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Not applicable.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{Not applicable.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Not applicable.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Not applicable.}
\end{enumerate}

\end{enumerate}

==> disclaimer.tex <==
\section*{Mistake in Theorem \ref{thm:softmax_rates} at submission time}
After main document deadline for submissions, we noticed that we overlooked a problem in the proof of Theorem \ref{thm:softmax_rates} that is encountered when the set of optimal actions is larger than 1 in some state. For the sake of transparency, we explain in the proof where this overlook happened.

Theorem \ref{thm:softmax_rates_mult} deals with the general setting, as described in the paper, but the bound is significantly worsen. Under the additional assumption \ass{8}:
\begin{enumerate}
    \item[] \ass{8}. The optimal policy is unique: $\forall s, \; q_\star(s,a_1)=q_\star(s,a_2)=v_\star(s)$ implies $a_1 = a_2$,
\end{enumerate}
Theorem \ref{thm:softmax_rates}, which is a corollary to Theorem \ref{thm:softmax_rates_mult}, provides efficient bounds that even improve the rate stated in the main document from $\mathcal{O}(|\mathcal{A}|^3)$ to $\mathcal{O}(|\mathcal{A}|)$).

We believe that the issue is not structural to the problem; it rather stems from our proof technique that relies on a sequence $x_t$ bounding $1-\sum_{a\in\mathcal{A}^{\mytop}_s}\pi_t(a_t|s)$ below, and then using this sequence to bound $X_t$ above, and these bounds cannot match when $|\mathcal{A}^{\mytop}_s| > 1$. However, it does not really matter whether $1-\sum_{a\in\mathcal{A}^{\mytop}_s}\pi_t(a_t|s)$ matches the lower or the upper bound, because the evolution of $x_t$ would auto-regulate to something in the form of efficient bounds. We did not find the solution in the limited time we had to fix the issue, but we are rather confident, or at least hope to find it by the rebuttal period.

In App. \ref{app:softmax-bounds}, we further compare \ass{8} with the setting used in \cite{mei2020global} that derives the only comparable theoretical result in the literature.

We would like to apologize to the reviewers for the time they might have lost on this issue.
